Rapid Trajectory Optimization Using C-FROST with Illustration on a Cassie-Series Dynamic Walking Biped

One of the big attractions of low-dimensional models for gait design has been the ability to compute solutions rapidly, whereas one of their drawbacks has been the difficulty in mapping the solutions back to the target robot. This paper presents a set of tools for rapidly determining solutions for ``humanoids'' without removing or lumping degrees of freedom. The main tools are (1) C-FROST, an open-source C++ interface for FROST, a direct collocation optimization tool; and (2) multi-threading. The results will be illustrated on a 20-DoF floating-base model for a Cassie-series bipedal robot through numerical calculations and physical experiments.

==> section_testbed.tex <==
\section{Testbed Model}
\label{sec:TestBed}

The results of the paper will be illustrated on the Cassie-series bipedal robot shown in Fig.~\ref{fig:cassie}.
%The robot's floating base model has 20 degrees of freedom (DOF), with seven joints in each leg with five of them actuated by electric motors through gearing and the other two joints are passive; instead, they are realized via a specially designed four-bar linkage with one bar being a leaf spring.
This underactuated robot's floating base model has 20 degrees of freedom (DOF). There are seven joints in each leg with five of them actuated by electric motors through gearing and the other two joints being passive where they are realized via a specially designed four-bar linkage with one bar being a leaf spring. 
% The robot is equipped with joint encoders and an inertial measurement unit (IMU).
When supported on one foot during walking, the robot is underactuated due to the narrow feet. The springs in the four-bar linkages also introduce additional underactuation.

Agility Robotics has released dynamic models of the robot in MuJuCo and in Gazebo \cite{AgilitySimsJune2018}. These models include the springs in the legs. To date, the control design done at Michigan on the Cassie robot has assumed these springs have infinite stiffness, i.e, rigid links, \cite{ACassieBlueYouTube2018} and this paper will do the same. The description of mechanical model of Cassie used in this paper is publicly released on GitHub\footnote{Available at \url{https://github.com/UMich-BipedLab/Cassie_Model}.}.

In this paper, we will use FROST to model and formulate a series of optimization problems for the Cassie robot corresponding to periodic walking, and then use C-FROST to rapidly generate these gaits in parallel. The optimization performance will be evaluated on multiple platforms---including remote cloud services---with different numbers of CPU cores. While the present paper is concerned with optimization of the open-loop model of Cassie, some of the designed gaits are implemented to demonstrate that they are physically realistic, and for that, a control policy is necessary. The control laws used in the simulations and experiments reported here are based on \cite{da20162d}.  The details on the selection of virtual constraints for the Cassie robot and how the physical constraints imposed for gait design relate to the physics of the robot will be given in a separate publication and the control code will be released on GitHub. To enhance our confidence that the presented optimization results are representative of what other users will find on their models, we have also run several of them on an 18-DOF exoskeleton model presented in \cite{Harib2018Feedback}. These results are not reported here.

